A Multimodal Approach to Heritage Preservation in the Context of Climate Change

Cultural heritage sites face accelerating degradation due to climate change, yet tradi- tional monitoring relies on unimodal analysis (visual inspection or environmental sen- sors alone) that fails to capture the complex interplay between environmental stres- sors and material deterioration. We propose a lightweight multimodal architecture that fuses sensor data (temperature, humidity) with visual imagery to predict degradation severity at heritage sites. Our approach adapts PerceiverIO with two key innovations: (1) simplified encoders (64D latent space) that prevent overfitting on small datasets (n=37 training samples), and (2) Adaptive Barlow Twins loss that encourages modality complementarity rather than redundancy. On data from Strasbourg Cathedral, our model achieves 76.9% accu- racy, a 43% improvement over standard multimodal architectures (VisualBERT, Trans- former) and 25% over vanilla PerceiverIO. Ablation studies reveal that sensor-only achieves 61.5% while image-only reaches 46.2%, confirming successful multimodal synergy. A systematic hyperparameter study identifies an optimal moderate correlation target ({\tau} =0.3) that balances align- ment and complementarity, achieving 69.2% accuracy compared to other {\tau} values ({\tau} =0.1/0.5/0.7: 53.8%, {\tau} =0.9: 61.5%). This work demonstrates that architectural sim- plicity combined with contrastive regularization enables effective multimodal learning in data-scarce heritage monitoring contexts, providing a foundation for AI-driven con- servation decision support systems.

==> PCJ-pagedegarde.tex <==
\makeatletter
\newgeometry{margin=2.54cm,top=2.54cm}
\thispagestyle{empty}

\vfill

\ifx\PDGauthors\undefined\let\PDGauthors\authors\fi

    \begin{minipage}[t]{.9\textwidth}
        \normalsize\setlength{\parskip}{3ex}
        \def\IsEqualContrib{\textsuperscript{$\#$,}\global\cdr@hasequalcontribtrue}

        {\raggedright\Huge\bf\@title\par}

        {\raggedright\LARGE\let\footnotesize=\normalsize\cdr@listauthors@footnotes\par}

%        {\Large Volume \textbf{\currentvolume} (\currentyear), article \thearticle}

        

        \bigskip{\huge\bf Abstract}\\[1ex]
        \normalsize{\setlength{\parskip}{0ex}\@abstract\par}

        \ifx\@empty\@keywords\else\textbf{Keywords:} \@keywords\par\fi

        \footnotesize\cdr@listaddresses@footnotes
        \ifcdr@hasequalcontrib,\quad\textsuperscript{$\#$}Equal contribution\par\fi
        
        \normalsize\textbf{Correspondence}\\
        {\url@sfstyle\url{\thePCIcorresp}}

    \end{minipage}


\vfill\restoregeometry

